Minimum R\'enyi Entropy Portfolios

Accounting for the non-normality of asset returns remains challenging in robust portfolio optimization. In this article, we tackle this problem by assessing the risk of the portfolio through the "amount of randomness" conveyed by its returns. We achieve this by using an objective function that relies on the exponential of R\'enyi entropy, an information-theoretic criterion that precisely quantifies the uncertainty embedded in a distribution, accounting for higher-order moments. Compared to Shannon entropy, R\'enyi entropy features a parameter that can be tuned to play around the notion of uncertainty. A Gram-Charlier expansion shows that it controls the relative contributions of the central (variance) and tail (kurtosis) parts of the distribution in the measure. We further rely on a non-parametric estimator of the exponential R\'enyi entropy that extends a robust sample-spacings estimator initially designed for Shannon entropy. A portfolio selection application illustrates that minimizing R\'enyi entropy yields portfolios that outperform state-of-the-art minimum variance portfolios in terms of risk-return-turnover trade-off.

==> ComonotonicLongProof.tex <==
\subsubsection{Counter-example to comonotonic additivity}\label{CounterExampleComonotonic}

This appendix details the counter-example to comonotonic additivity of $H_\alpha^{\text{exp}}$ as mentioned in section \ref{subadditivity}. We give a counter-example for $\alpha=1$, i.e. the exponential Shannon entropy.  

Two random variables $X,Y$ are comonotonic when $Y$ can be written as $F(X)$ where $F$ is a continuous and strictly increasing function.\footnote{The case where $F$ is decreasing, i.e.\ perfect negative dependence, can not be treated because $X+Y = X + F(X)$ does not necessarily have an inverse}. Let's denote $G(x) \coloneqq x + F(x)$, which is also strictly increasing and so invertible, and let's denote $H(x)$ its inverse. Then, the cdf of $X+Y=G(X)$ is given by
\begin{equation*}
F_{X+Y}(x) = \mathbb{P}(G(X) \leqslant x) = \mathbb{P}(X \leqslant H(x))=F_X(H(x)),
\end{equation*}
and its pdf reads
\begin{equation*}
f_{X+Y}(x) = \frac{f_X(H(x))}{G'(H(x))}.
\end{equation*}
As a result, $H_1^{\text{exp}}(X+Y)$ becomes
\begin{equation*}
H_1^{\text{exp}}(X+Y) = \text{exp} \Bigg(-\int \frac{f_X(H(x))}{G'(H(x))} \hspace{0.05cm}\text{ln}\hspace{0.02cm}\frac{f_X(H(x))}{G'(H(x))} \hspace{0.05cm} dx\Bigg).
\end{equation*}
By making a change of variable $z=H(x)$, we get $dx = \frac{dz}{H'(x)} = \frac{dz}{H'(H^{-1}(z))} = (H^{-1})'(z) dz = G'(z)dz$, leading to 

\begin{align*}
H_1^{\text{exp}}(X+Y) &= \text{exp} \Bigg(-\int \bigg( \frac{f_X(z)}{G'(z)} \hspace{0.05cm}\text{ln}\hspace{0.02cm}\frac{f_X(z)}{G'(z)} \bigg) G'(z) dz\Bigg) \\
&= \text{exp} \Bigg(-\int f_X(z) \hspace{0.05cm}\text{ln}\hspace{0.02cm}\frac{f_X(z)}{G'(z)} \hspace{0.05cm} dz\Bigg)
\\
&= H_1^{\text{exp}}(X) \hspace{0.05cm} \text{exp}\Bigg(\int f_X(z) \hspace{0.05cm} \text{ln}\hspace{0.05cm} G'(z) \hspace{0.05cm} dz\Bigg) \\
&= H_1^{\text{exp}}(X) \hspace{0.05cm} \text{exp} \Big( \mathbb{E}\big[\text{ln} \hspace{0.05cm} G'(X)\big]\Big) \\
&= H_1^{\text{exp}}(X) \hspace{0.05cm} \text{exp} \Big( \mathbb{E}\big[\text{ln} (1+F'(X))\big]\Big).
\end{align*}
Based on similar reasoning, we can show that
\begin{equation*}
H_1^{\text{exp}}(Y) = H_1^{\text{exp}}(X) \hspace{0.05cm} \text{exp} \Big( \mathbb{E}\big[\text{ln} \hspace{0.05cm} F'(X)\big]\Big),
\end{equation*}
meaning that additivity amounts to showing that 
\begin{equation}\label{additivitycondition}
\text{exp}\Big(\mathbb{E}\big[\text{ln}(1+F'(X))\big]\Big) = 1 + \text{exp}\Big(\mathbb{E}\big[\text{ln}(F'(X))\big]\Big)
\end{equation}

Let's now show a counter-example to \eqref{additivitycondition} where the left-hand side is higher than the right-hand side, i.e. where $H_1^{\text{exp}}$ is super-additive. Because $F'(X)$ has to be a positive random variable (since $F$ is strictly increasing), we consider the case where $F'(X):=\zeta\sim Exp(1)$.
Define $W:=\ln(1+\zeta)$ and $Z:=\ln\zeta$. To have additivity, we have to show that 
\begin{equation}\label{additiveExp}
e^{\mathbb{E}[W]} = 1+e^{\mathbb{E}[Z]}.
\end{equation}
The cdf of $W$ is given by
\begin{align*}
F_W(x)
&= \mathbb{P}(\zeta \leqslant e^x - 1) 
=1-e^{1-e^x},
\end{align*}
for $x \geqslant 0$ 
and 0 otherwise, and so its pdf reads
\begin{equation}\label{pdfW}
f_W(x) = e^{1+x-e^x}\; .
\end{equation}
A similar reasoning for $Z$ yields
\begin{equation}\label{pdfZ}
f_Z(x) = e^{x-e^x}
\end{equation}
for $x\in\mathbb{R}$ (because this time the condition is $e^x \geqslant 0$). 

We can now compute the expectations. From \eqref{pdfW}, $\mathbb{E}[W]$ is given by the following integral:
\begin{equation*}
\begin{aligned}
\mathbb{E}[W] 
&= e \int_0^{\infty} xe^{x-e^x}dx.
\end{aligned}
\end{equation*}
A change of variable $z=e^x$ yields
\begin{equation*}
\begin{aligned}
\mathbb{E}[W]
&= e \int_1^{\infty} \ln z \hspace{0.05cm} e^{-z} dz,
\end{aligned}
\end{equation*}
which, by integration by parts, becomes
\begin{equation*}
\begin{aligned}
\mathbb{E}[W] &= e\Bigg(\underbrace{\Big[\ln (z)e^{-z}\Big]_1^{\infty}}_\text{= 0} \hspace{0.05cm} \int_1^{\infty} \frac{e^{-z}}{z}dz\Bigg) \\
&= e \hspace{0.05cm} \Gamma(0,1) \approx 0.596,
\end{aligned}
\end{equation*}
where $ \Gamma(s,x)=\int_x^\infty t^{s-1}e^{-t}dt$ is the upper incomplete Gamma function. The expectation $\mathbb{E}[Z]$ does not yield such a result but, from \eqref{pdfZ}, can be found by numerical integration of $xf_Z(x)$ for $x \in \mathbb{R}$, which yields $\mathbb{E}[W] \approx -0.578$, with an error bound of less than $10^{-6}$. 

Finally, we have that
\begin{equation*}
e^{\mathbb{E}[W]} \approx 1.815 \geq 1.561 \approx 1+e^{\mathbb{E}[Z]},
\end{equation*}
hence violating equality \eqref{additiveExp} and therefore providing a counter-example to comonotonic additivity. 
